Beyond Borders: Investigating Cross-Jurisdiction Transfer in Legal Case Summarization

Legal professionals face the challenge of managing an overwhelming volume of lengthy judgments, making automated legal case summarization crucial. However, prior approaches mainly focused on training and evaluating these models within the same jurisdiction. In this study, we explore the cross-jurisdictional generalizability of legal case summarization models.Specifically, we explore how to effectively summarize legal cases of a target jurisdiction where reference summaries are not available. In particular, we investigate whether supplementing models with unlabeled target jurisdiction corpus and extractive silver summaries obtained from unsupervised algorithms on target data enhances transfer performance. Our comprehensive study on three datasets from different jurisdictions highlights the role of pre-training in improving transfer performance. We shed light on the pivotal influence of jurisdictional similarity in selecting optimal source datasets for effective transfer. Furthermore, our findings underscore that incorporating unlabeled target data yields improvements in general pre-trained models, with additional gains when silver summaries are introduced. This augmentation is especially valuable when dealing with extractive datasets and scenarios featuring limited alignment between source and target jurisdictions. Our study provides key insights for developing adaptable legal case summarization systems, transcending jurisdictional boundaries.

==> text/segment-tab.tex <==
\begin{table*}[!ht]
\caption{Segment-wise ROUGE-L Recall scores on the UK-Abs dataset. BGA, Jud., Rea. indicate ‘Background to the Appeal’, ‘Judgement’, and ‘Reasons for Judgement’ respectively. \textcolor{cyan}{EDIT: New table in Table 11}}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\hspace{2cm}\textbf{Source \textrightarrow}}                                                                                & \multicolumn{3}{c|}{\textbf{IN-Abs}}                                                                  & \multicolumn{3}{c|}{\textbf{BVA-Ext}}                                                                     \\ \hline
\multicolumn{2}{|c|}{\textbf{Model Config}}                                                                         & {\hspace{0.22cm}\textbf{BGA}\hspace{0.22cm}} & \hspace{0.22cm}{\textbf{Jud.}}\hspace{0.22cm} & \hspace{0.22cm}\textbf{Rea.}\hspace{0.22cm} & \hspace{0.22cm}{\textbf{BGA}}\hspace{0.22cm} & \hspace{0.22cm}{\textbf{Jud.}}\hspace{0.22cm} & \hspace{0.22cm}\textbf{Rea.}\hspace{0.22cm} \\ \hline
{\multirow{4}{*}{BART}}      &             & {0.319}               & {0.488}              & 0.283            & {0.315}               & {0.449}              & 0.295            \\ \cline{2-8} 
{}                           & GRL         & {0.377}               & {0.528}              & 0.34             & {0.318}               & {0.452}              & 0.301            \\ \cline{2-8} 
{}                           & Silver (CS) & {0.337}               & {0.491}              & 0.281            & {0.334}               & {0.471}              & 0.284            \\ \cline{2-8} 
{}                           & Silver(MMR) & {0.348}               & {0.492}              & 0.293            & {0.338}               & {0.471}              & 0.302            \\ \hline
{\multirow{4}{*}{BART-BERT}} &             & {0.312}               & {0.474}              & 0.266            & {0.309}               & {0.445}              & 0.281            \\ \cline{2-8} 
{}                           & GRL         & {0.337}               & {0.493}              & 0.294            & {0.313}               & {0.45}               & 0.286            \\ \cline{2-8} 
{}                           & Silver (CS) & {0.329}               & {0.481}              & 0.266            & {0.332}               & {0.468}              & 0.271            \\ \cline{2-8} 
{}                           & Silver(MMR) & {0.337}               & {0.479}              & 0.286            & {0.334}               & {0.47}               & 0.294            \\ \hline
\end{tabular}
\label{segment}
\end{table*}

==> text/tab-RQ1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!ht]
\centering
\caption{ROUGE-1, 2 and L F-scores of all methods across three datasets. Each test dataset is represented by a column, while the training dataset used for supervision is indicated in the "Train" column, if applicable.}
\scalebox{0.9}{
\begin{tabular}{|c|c|c|c|c|}
\hline
{\textbf{}}                      & {\textbf{Test} \textrightarrow}      & {\textbf{UK-Abs}}      & {\textbf{IN-Abs}}      & \textbf{BVA-Ext}         \\ \hline
\hspace{0.2cm}{\textbf{Model}} \hspace{0.2cm}                & \hspace{0.25cm}{\textbf{Train \textdownarrow}}\hspace{0.25cm} & \hspace{0.35cm}{\textbf{R-1/R-2/R-L}}\hspace{0.35cm} & \hspace{0.35cm}{\textbf{R-1/R-2/R-L}}\hspace{0.35cm} & \hspace{0.35cm}\textbf{R-1/R-2/R-L}\hspace{0.35cm} \\ \hline
\multicolumn{5}{|c|}{Unsupervised, Domain-Agnostic, Extractive Models}                                                                                                                                    \\ \hline
{LexRank}                        & {None}           & {0.483/0.225/0.427}    & {0.523/0.286/0.459}    & 0.546/0.341/0.356    \\ \hline
{LSA}                            & {None}           & {0.419/0.159/0.361}    & {0.479/0.236/0.410}     & 0.516/0.281/0.308    \\ \hline
{Luhn}                           & {None}           & {0.501/0.194/0.435}    & {0.522/0.270/0.454}     & 0.530/0.340/0.363      \\ \hline
{Reduction}                      & {None}           & {0.551/0.228/0.484}    & {0.537/0.300/0.473}      & 0.534/0.373/0.394    \\ \hline
\multicolumn{5}{|c|}{Unsupervised, Domain-Specific, Extractive Models}                                                                                                                                    \\ \hline
{CaseSummarizer}                 & {None}           & {0.596/0.251/0.519}    & {0.599/0.300/0.517}      & 0.436/0.181/0.346    \\ \hline
{LetSum}                         & {None}           & {0.400/0.139/0.360}       & {0.405/0.144/0.362}    & 0.391/0.156/0.298    \\ \hline
{MMR}                            & {None}           & {0.595/0.248/0.567}    & {0.581/0.296/0.548}    & 0.514/0.267/0.384    \\ \hline
\multicolumn{5}{|c|}{Supervised, Domain-Agnostic, Extractive Models}                                                                                                                                      \\ \hline
{\multirow{3}{*}{SummaRuNNer}}   & {UK-Abs}         & {0.459/0.223/0.408}    & {0.473/0.230/0.410}      & 0.497/0.368/0.405    \\ \cline{2-5} 
{}                               & {IN-Abs}         & {0.487/0.225/0.430}     & {0.536/0.303/0.471}    & 0.455/0.273/0.327    \\ \cline{2-5} 
{}                               & {BVA-Ext}            & {0.430/0.196/0.378}     & {0.438/0.199/0.374}    & 0.516/0.423/0.453    \\ \hline
\multicolumn{5}{|c|}{Pre-trained, Domain-Agnostic/Specific, Abstractive/Hybrid Models}                                                                                                                    \\ \hline
{BART}                           & {Vanilla}        & {0.602/0.243/0.517}    & {0.570/0.268/0.486}     & 0.482/0.301/0.344    \\ \hline
{Legal-Pegasus}                  & {Vanilla}        & {0.590/0.242/0.517}     & {0.601/0.302/0.522}    & 0.493/0.246/0.296    \\ \hline
{Legal-LED}                      & {Vanilla}        & {0.272/0.089/0.240}     & {0.342/0.108/0.292}    & 0.447/0.174/0.232    \\ \hline
{BERT-BART}                      & {Vanilla}        & {0.586/0.227/0.501}    & {0.566/0.266/0.482}    & 0.492/0.307/0.349    \\ \hline
\multicolumn{5}{|c|}{Fine-tuned, Domain-Agnostic, Abstractive Models}                                                                                                                                     \\ \hline
{\multirow{3}{*}{BART}}          & {UK-Abs}         & {0.627/0.272/0.543}    & {0.608/0.311/0.522}    & 0.555/0.334/0.340    \\ \cline{2-5} 
{}                               & {IN-Abs}         & {0.615/0.255/0.532}    & {0.625/0.337/0.548}    & 0.481/0.226/0.306    \\ \cline{2-5} 
{}                               & {BVA-Ext}            & {0.598/0.242/0.519}    & {0.581/0.277/0.503}    & 0.605/0.435/0.472    \\ \hline
\multicolumn{5}{|c|}{Fine-tuned, Domain-Specific, Abstractive Models}                                                                                                                                     \\ \hline
{\multirow{3}{*}{Legal-Pegasus}} & {UK-Abs}         & {0.624/0.271/0.541}    & {0.615/0.323/0.532}    & 0.528/0.308/0.343    \\ \cline{2-5} 
{}                               & {IN-Abs}         & {0.617/0.259/0.533}    & {0.629/0.342/0.547}    & 0.518/0.292/0.336    \\ \cline{2-5} 
{}                               & {BVA-Ext}            & {0.596/0.247/0.522}    & {0.601/0.303/0.522}    & 0.603/0.424/0.453    \\ \hline
{\multirow{3}{*}{Legal-LED}}     & {UK-Abs}         & {0.541/0.245/0.467}    & {0.493/0.231/0.418}    & 0.547/0.323/0.321    \\ \cline{2-5} 
{}                               & {IN-Abs}         & {0.556/0.239/0.479}    & {0.555/0.301/0.480}     & 0.541/0.315/0.339    \\ \cline{2-5} 
{}                               & {BVA-Ext}            & {0.265/0.116/0.233}    & {0.337/0.156/0.289}    & 0.552/0.353/0.379    \\ \hline
\multicolumn{5}{|c|}{Fine-tuned, Domain-Agnostic, Hybrid Models}                                                                                                                                          \\ \hline
{\multirow{3}{*}{BERT-BART}}     & {UK-Abs}         & {0.615/0.260/0.529}     & {0.600/0.305/0.513}      & 0.552/0.334/0.342    \\ \cline{2-5} 
{}                               & {IN-Abs}         & {0.599/0.244/0.515}    & {0.620/0.330/0.541}      & 0.482/0.229/0.308    \\ \cline{2-5} 
{}                               & {BVA-Ext}            & {0.590/0.235/0.508}     & {0.580/0.279/0.501}     & 0.602/0.427/0.465    \\ \hline
\end{tabular}}
\end{table*}


==> text/tab-RQ1v2.tex <==
\begin{table*}[!ht]
\centering
\caption{ROUGE-L F scores (R-L) and BERT Score (BS) of all methods across three datasets. Each test dataset is represented by a column, while the training dataset used for supervision is indicated in the Train column, if applicable. \textcolor{cyan}{\textbf{EDIT : New variants added table 5. 6. I prefer 6 with removing legal-LED}.}}
\label{RQ1}
\scalebox{0.9}{
\begin{tabular}{|c|c|c|c|c|}
\hline
{\textbf{}}                      & {\textbf{Test} \textrightarrow}      & {\textbf{UK-Abs}}      & {\textbf{IN-Abs}}      & \textbf{BVA-Ext}         \\ \hline
\hspace{0.7cm}{\textbf{Model}} \hspace{0.7cm}                & \hspace{0.5cm}{\textbf{Train \textdownarrow}}\hspace{0.5cm} & \hspace{0.55cm}{\textbf{R-L/BS}}\hspace{0.55cm} & \hspace{0.55cm}{\textbf{R-L/BS}}\hspace{0.55cm} & \hspace{0.55cm}\textbf{R-L/BS}\hspace{0.55cm} \\ \hline
\multicolumn{5}{|c|}{Unsupervised, Domain-Agnostic, Extractive Models}                                                                                                                      \\ \hline
{LexRank}                        & {None}           & {0.427/\textbf{0.836}}     & {0.439/\textbf{0.850}}     & 0.356/0.862      \\ \hline
{LSA}                            & {None}           & {0.361/0.823}     & {0.410/0.841}     & 0.308/0.854      \\ \hline
{Luhn}                           & {None}           & {0.435/0.828}     & {0.414/0.843}     & 0.353/0.860      \\ \hline
{Reduction}                      & {None}           & {0.424/0.829}     & {0.423/0.847}     & 0.364/\textbf{0.865}      \\ \hline
\multicolumn{5}{|c|}{Unsupervised, Domain-Specific, Extractive Models}                                                                                                                      \\ \hline
{CaseSummarizer}                 & {None}           & {0.443/0.835}     & {0.476/0.836}     & \textbf{0.386}/0.829      \\ \hline
{LetSum}                         & {None}           & {0.361/0.772}     & {0.362/0.797}     & 0.298/0.807      \\ \hline
{MMR}                            & {None}           & {\textbf{0.467}/0.834}     & {\textbf{0.485}/0.847}     & 0.384/0.825      \\ \hline \hline
\multicolumn{5}{|c|}{Supervised, Domain-Agnostic, Extractive Models}                                                                                                                        \\ \hline
{\multirow{3}{*}{SummaRuNNer}}   & {UK-Abs}         & {0.408/0.845}     & {0.410/0.832}     & 0.405/0.861      \\ \cline{2-5} 
{}                               & {IN-Abs}         & {0.430/0.834}     & {0.471/0.849}     & 0.327/0.846      \\ \cline{2-5} 
{}                               & {BVA-Ext}        & {0.378/0.782}      & {0.374/0.839}     & 0.453/0.876      \\ \hline
\multicolumn{5}{|c|}{Domain-Agnostic, Abstractive Models}                                                                                                                                   \\ \hline
{\multirow{4}{*}{BART}}          & {Vanilla}        & {0.517/0.833}     & {0.486/0.839}     & 0.334/0.841      \\ \cline{2-5} 
{}                               & {UK-Abs}         & {0.543/0.844}     & {0.522/0.845}     & 0.341/0.842      \\ \cline{2-5} 
{}                               & {IN-Abs}         & {0.532/0.837}     & {0.548/0.851}     & 0.306/0.834      \\ \cline{2-5} 
{}                               & {BVA-Ext}        & {0.519/0.835}     & {0.503/0.840}     & 0.472/0.881      \\ \hline
\multicolumn{5}{|c|}{Domain-Specific, Abstractive Models}                                                                                                                                   \\ \hline
{\multirow{4}{*}{Legal-Pegasus}} & {Vanilla}        & {0.517/0.831}     & {0.522/0.841}     & 0.386/0.830      \\ \cline{2-5} 
{}                               & {UK-Abs}         & {0.541/0.838}     & {0.532/0.847}     & 0.451/0.861      \\ \cline{2-5} 
{}                               & {IN-Abs}         & {0.533/0.838}     & {0.547/0.850}     & 0.434/0.854      \\ \cline{2-5} 
{}                               & {BVA-Ext}        & {0.522/0.834}     & {0.522/0.842}     & 0.473/0.878      \\ \hline
{\multirow{4}{*}{Legal-LED}}     & {Vanilla}        & {0.240/0.821}     & {0.292/0.812}     & 0.232/0.832      \\ \cline{2-5} 
{}                               & {UK-Abs}         & {0.468/0.831}     & {0.418/0.838}     & 0.321/0.834      \\ \cline{2-5} 
{}                               & {IN-Abs}         & {0.479/0.832}     & {0.480/0.840}     & 0.339/0.831      \\ \cline{2-5} 
{}                               & {BVA-Ext}        & {0.233/0.817}     & {0.289/0.812}     & 0.379/0.841      \\ \hline
\multicolumn{5}{|c|}{Domain-Agnostic, Hybrid Models}                                                                                                                                        \\ \hline
{\multirow{4}{*}{BERT-BART}}     & {Vanilla}        & {0.501/0.836}     & {0.482/0.838}     & 0.329/0.844      \\ \cline{2-5} 
{}                               & {UK-Abs}         & {0.529/0.845}     & {0.513/0.846}     & 0.342/0.842      \\ \cline{2-5} 
{}                               & {IN-Abs}         & {0.515/0.837}     & {0.541/0.851}     & 0.308/0.836      \\ \cline{2-5} 
{}                               & {BVA-Ext}        & {0.508/0.836}     & {0.501/0.839}     & 0.465/0.880      \\ \hline
\end{tabular}}
\end{table*}

==> text/tab-RQ1v3.tex <==
\begin{table*}[!ht]
\centering
\caption{ROUGE-L F scores (R-L) and BERT Score (BS) of all methods across three datasets. Each test dataset is represented by a column, while the training dataset used for supervision is indicated in the Train column, if applicable.}
\scalebox{0.9}{
\begin{tabular}{|c|c|c|c|c|}
\hline
{\textbf{}}                      & {\textbf{Test} \textrightarrow}      & {\textbf{UK-Abs}}      & {\textbf{IN-Abs}}      & \textbf{BVA-Ext}         \\ \hline
\hspace{0.7cm}{\textbf{Model}} \hspace{0.7cm}                & \hspace{0.5cm}{\textbf{Train \textdownarrow}}\hspace{0.5cm} & \hspace{0.55cm}{\textbf{R-L/BS}}\hspace{0.55cm} & \hspace{0.55cm}{\textbf{R-L/BS}}\hspace{0.55cm} & \hspace{0.55cm}\textbf{R-L/BS}\hspace{0.55cm} \\ \hline
\multicolumn{5}{|c|}{Unsupervised, Extractive Models}                                                                                                                      \\ \hline
{LexRank}                        & {-}           & {0.427/\textbf{0.836}}     & {0.439/\textbf{0.850}}     & 0.356/0.862      \\ \hline
{LSA}                            & {-}           & {0.361/0.823}     & {0.410/0.841}     & 0.308/0.854      \\ \hline
{Luhn}                           & {-}           & {0.435/0.828}     & {0.414/0.843}     & 0.353/0.860      \\ \hline
{Reduction}                      & {-}           & {0.424/0.829}     & {0.423/0.847}     & 0.364/\textcolor{magenta} {\textbf{0.865}}     \\ \hline
%\multicolumn{5}{|c|}{Unsupervised, Domain-Specific, Extractive Models}                                                                                                                      \\ \hline
{CaseSummarizer}                 & {-}           & {0.443/0.835}     & {0.476/0.836}     & \textbf{0.386}/0.829      \\ \hline
{LetSum}                         & {-}           & {0.361/0.772}     & {0.362/0.797}     & 0.298/0.807      \\ \hline
{MMR}                            & {-}           & {\textbf{0.467}/0.834}     & {\textbf{0.485}/0.847}     & 0.384/0.825      \\ \hline 
\multicolumn{5}{|c|}{Supervised,  Extractive Models}                                                                                                                        \\ \hline
{\multirow{3}{*}{SummaRuNNer}}   & {UK-Abs}         & {-}     & {\textbf{0.410}/\textbf{0.832}}     & \textbf{0.405}/\textbf{0.861}      \\ \cline{2-5} 
{}                               & {IN-Abs}         & {\textbf{0.430}/\textbf{0.834}}     & {-}     & 0.327/0.846      \\ \cline{2-5} 
{}                               & {BVA-Ext}        & {0.378/0.782}      & {0.374/0.839}     & -     \\ \hline
\multicolumn{5}{|c|}{Abstractive \& Hybrid Models}                                                                                                                                   \\ \hline
{\multirow{4}{*}{BART}}          & {-}        & {0.517/0.833}     & {0.486/0.839}     & 0.324/0.841      \\ \cline{2-5} 
{}                               & {UK-Abs}         & {-}     & {\textbf{0.522}/\textbf{0.845}}     & \textbf{0.341}/\textbf{0.842}      \\ \cline{2-5} 
{}                               & {IN-Abs}         & {\textbf{0.532}/\textbf{0.837}}     & {-}     & 0.306/0.834      \\ \cline{2-5} 
{}                               & {BVA-Ext}        & {0.519/0.835}     & {0.503/0.840}     & -     \\ \hline
%\multicolumn{5}{|c|}{Domain-Specific, Abstractive Models}                                                                                                                                   \\ \hline
{\multirow{4}{*}{Legal-Pegasus}} & {-}        & {0.517/0.831}     & {0.522/0.841}     & 0.386/0.830      \\ \cline{2-5} 
{}                               & {UK-Abs}         & {-}     & 
\textcolor{magenta} {\textbf{0.532}}/ 
\textcolor{magenta} {\textbf{0.847}} & 
\textcolor{magenta} {\textbf{0.451}}/\textbf{0.861}      \\ \cline{2-5} 
{}                               & {IN-Abs}         & 
\textcolor{magenta} {\textbf{0.533}}/ 
\textcolor{magenta} {\textbf{0.838}} & {-}     & 0.434/0.854      \\ \cline{2-5} 
{}                               & {BVA-Ext}        & {0.522/0.834}     & {0.522/0.842}     & -      \\ \hline
{\multirow{4}{*}{Legal-LED}}     & {-}        & {0.240/0.821}     & {0.292/0.812}     & 0.232/0.832      \\ \cline{2-5} 
{}                               & {UK-Abs}         & {-}     & {\textbf{0.418}/\textbf{0.838}}     & 0.321/\textbf{0.834}      \\ \cline{2-5} 
{}                               & {IN-Abs}         & {\textbf{0.479}/\textbf{0.832}}     & {-}     & \textbf{0.339}/0.831     \\ \cline{2-5} 
{}                               & {BVA-Ext}        & {0.233/0.817}     & {0.289/0.812}     & -      \\ \hline
%\multicolumn{5}{|c|}{Domain-Agnostic, Hybrid Models}                                                                                                                                        \\ \hline
{\multirow{4}{*}{BERT-BART}}     & {-}        & {0.501/0.836}     & {0.482/0.838}     & 0.329/0.844      \\ \cline{2-5} 
{}                               & {UK-Abs}         & {-}     & {\textbf{0.513/0.846}}     & \textbf{0.342/0.842}      \\ \cline{2-5} 
{}                               & {IN-Abs}         & {\textbf{0.515/0.837}}     & {-}     & 0.308/0.836      \\ \cline{2-5} 
{}                               & {BVA-Ext}        & {0.508/0.836}     & {0.501/0.839}     & -     \\ \hline
\end{tabular}}
\label{RQ1}
\end{table*}

==> text/tab-RQ2-3v1.tex <==
\begin{table*}[]
\scalebox{0.7}{
\centering
\begin{tabular}%{|p{1.2cm}|p{1.8cm}|p{2.4cm}|p{3cm}|p{2.4cm}|p{3cm}|p{2.4cm}|p{3cm}|}
{|c||c|c|c||c|c||c|c|c||c|c|}
\hline
\textbf{}                                                                  & \hspace{2cm} & \multicolumn{2}{c|}{\textbf{UK-Abs}}                                & \multicolumn{2}{c|}{\textbf{IN-Abs}}                                & \multicolumn{2}{c|}{\textbf{BVA}}                                   \\ \hline
\hspace{0.1cm} \textbf{Model}          \hspace{0.1cm}                                                   &           & \multicolumn{1}{c|}{\hspace{0.2cm} \textbf{Train}\hspace{0.2cm}}          &  \hspace{0.3cm} \textbf{R-1/R-2/R-L}\hspace{0.3cm}  & \multicolumn{1}{c|}{\hspace{0.2cm}\textbf{Train}\hspace{0.2cm}}          & \hspace{0.3cm}\textbf{R-1/R-2/R-L}\hspace{0.3cm} & \multicolumn{1}{c|}{\hspace{0.2cm}\textbf{Train}\hspace{0.2cm}}          &  \hspace{0.3cm}  \textbf{R-1/R-2/R-L} \hspace{0.3cm} \\ \hline
\multirow{9}{*}{BART}                                                      &           & \multicolumn{1}{c|}{UK-Abs }                  & 0.627/0.272/0.543    & \multicolumn{1}{c|}{IN-Abs}                  & 0.625/0.337/0.548   & \multicolumn{1}{c|}{BVA}                     & 0.605/0.435/0.472    \\ \cline{2-8} 
                                                                           &           & \multicolumn{1}{c|}{\multirow{4}{*}{BVA}}    & 0.598/0.242/0.519    & \multicolumn{1}{c|}{\multirow{4}{*}{BVA}}    & 0.581/0.277/0.503    & \multicolumn{1}{c|}{\multirow{4}{*}{IN-Abs}} & 0.481/0.226/0.306    \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & GRL       & \multicolumn{1}{c|}{}                        & 0.604/0.243/0.544    & \multicolumn{1}{c|}{}                        & 0.581/0.278/0.513    & \multicolumn{1}{c|}{}                        & 0.524/0.294/0.44     \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & Sil. (CS) & \multicolumn{1}{c|}{}                        & 0.608/0.248/0.523    & \multicolumn{1}{c|}{}                        & //                   & \multicolumn{1}{c|}{}                        & 0.562/0.372/0.491    \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & Sil.(MMR) & \multicolumn{1}{c|}{}                        & //                   & \multicolumn{1}{c|}{}                        & 0.585/0.284/0.5      & \multicolumn{1}{c|}{}                        & //                   \\ \cline{2-8} 
                                                                           &           & \multicolumn{1}{c|}{\multirow{4}{*}{IN-Abs}} & 0.615/0.255/0.532    & \multicolumn{1}{c|}{\multirow{4}{*}{UK-Abs}} & 0.608/0.311/0.522    & \multicolumn{1}{c|}{\multirow{4}{*}{UK-Abs}} & 0.555/0.334/0.34     \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & GRL       & \multicolumn{1}{c|}{}                        & 0.62/0.264/0.536     & \multicolumn{1}{c|}{}                        & 0.614/0.316/0.526    & \multicolumn{1}{c|}{}                        & 0.553/0.336/0.46     \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & Sil. (CS) & \multicolumn{1}{c|}{}                        & 0.61/0.253/0.525     & \multicolumn{1}{c|}{}                        & //                   & \multicolumn{1}{c|}{}                        & //                   \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & Sil.(MMR) & \multicolumn{1}{c|}{}                        & //                   & \multicolumn{1}{c|}{}                        & 0.597/0.29/0.507     & \multicolumn{1}{c|}{}                        & 0.556/0.342/0.476    \\ \hline
\multirow{9}{*}{\begin{tabular}[c]{@{}l@{}}BERT-\\ BART\end{tabular}}      &           & \multicolumn{1}{c|}{UK-Abs}                  & 0.615/0.26/0.529     & \multicolumn{1}{c|}{IN-Abs}                  & 0.62/0.33/0.541      & \multicolumn{1}{c|}{BVA}                     & 0.602/0.427/0.465    \\ \cline{2-8} 
                                                                           &           & \multicolumn{1}{c|}{\multirow{4}{*}{BVA}}    & 0.59/0.235/0.508     & \multicolumn{1}{c|}{\multirow{4}{*}{BVA}}    & 0.58/0.279/0.501     & \multicolumn{1}{c|}{\multirow{4}{*}{IN-Abs}} & 0.482/0.229/0.308    \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & GRL       & \multicolumn{1}{c|}{}                        & 0.595/0.238/0.522    & \multicolumn{1}{c|}{}                        & 0.575/0.27/0.502     & \multicolumn{1}{c|}{}                        & 0.523/0.293/0.44     \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & Sil. (CS) & \multicolumn{1}{c|}{}                        & //                   & \multicolumn{1}{c|}{}                        & //                   & \multicolumn{1}{c|}{}                        & 0.564/0.373/0.493    \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & Sil.(MMR) & \multicolumn{1}{c|}{}                        & 0.594/0.238/0.517    & \multicolumn{1}{c|}{}                        & 0.585/0.278/0.499    & \multicolumn{1}{c|}{}                        & //                   \\ \cline{2-8} 
                                                                           &           & \multicolumn{1}{c|}{\multirow{4}{*}{IN-Abs}} & 0.599/0.244/0.515    & \multicolumn{1}{c|}{\multirow{4}{*}{UK-Abs}} & 0.6/0.305/0.513      & \multicolumn{1}{c|}{\multirow{4}{*}{UK-Abs}} & 0.552/0.334/0.342    \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & GRL       & \multicolumn{1}{c|}{}                        & 0.604/0.251/0.52     & \multicolumn{1}{c|}{}                        & 0.607/0.308/0.522    & \multicolumn{1}{c|}{}                        & 0.554/0.336/0.461    \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & Sil. (CS) & \multicolumn{1}{c|}{}                        & 0.597/0.24/0.511     & \multicolumn{1}{c|}{}                        & //                   & \multicolumn{1}{c|}{}                        & //                   \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & Sil.(MMR) & \multicolumn{1}{c|}{}                        & //                   & \multicolumn{1}{c|}{}                        & 0.595/0.291/0.505    & \multicolumn{1}{c|}{}                        & 0.556/0.343/0.477    \\ \hline
\multirow{9}{*}{\begin{tabular}[c]{@{}l@{}}Legal-\\ Pegasus\end{tabular}} &           & \multicolumn{1}{c|}{UK-Abs}                  & 0.624/0.271/0.541    & \multicolumn{1}{c|}{IN-Abs}                  & 0.629/0.342/0.547    & \multicolumn{1}{c|}{BVA}                     & 0.503/0.264/0.305    \\ \cline{2-8} 
                                                                           &           & \multicolumn{1}{c|}{\multirow{4}{*}{BVA}}    & 0.596/0.247/0.522    & \multicolumn{1}{c|}{\multirow{4}{*}{BVA}}    & 0.601/0.303/0.522    & \multicolumn{1}{c|}{\multirow{4}{*}{IN-Abs}} & 0.518/0.292/0.434    \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & GRL       & \multicolumn{1}{c|}{}                        & 0.599/0.235/0.517    & \multicolumn{1}{c|}{}                        & 0.609/0.301/0.523    & \multicolumn{1}{c|}{}                        & 0.403/0.154/0.326    \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & Sil. (CS) & \multicolumn{1}{c|}{}                        & 0.609/0.245/0.524    & \multicolumn{1}{c|}{}                        & 0.598/0.295/0.513    & \multicolumn{1}{c|}{}                        & //                   \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & Sil.(MMR) & \multicolumn{1}{c|}{}                        & //                   & \multicolumn{1}{c|}{}                        & //                   & \multicolumn{1}{c|}{}                        & 0.546/0.335/0.465    \\ \cline{2-8} 
                                                                           &           & \multicolumn{1}{c|}{\multirow{4}{*}{IN-Abs}} & 0.617/0.259/0.533    & \multicolumn{1}{c|}{\multirow{4}{*}{UK-Abs}} & 0.615/0.323/0.532    & \multicolumn{1}{c|}{\multirow{4}{*}{UK-Abs}} & 0.528/0.308/0.451    \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & GRL       & \multicolumn{1}{c|}{}                        & 0.609/0.235/0.528    & \multicolumn{1}{c|}{}                        & 0.611/0.297/0.524    & \multicolumn{1}{c|}{}                        & 0.485/0.242/0.394    \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & Sil. (CS) & \multicolumn{1}{c|}{}                        & 0.622/0.253/0.536    & \multicolumn{1}{c|}{}                        & //                   & \multicolumn{1}{c|}{}                        & //                   \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
                                                                           & Sil.(MMR) & \multicolumn{1}{c|}{}                        & //                   & \multicolumn{1}{c|}{}                        & 0.608/0.309/0.526    & \multicolumn{1}{c|}{}                        & 0.546/0.329/0.469    \\ \hline
\end{tabular}}
\end{table*}

==> text/tab-RQ2-3v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!ht]
\centering
\caption{ROUGE-1, 2 and L F-scores of three abstractive models trained under various configurations. Each test (target) dataset is represented by a column, while the training dataset (source) is presented in the "Train" column. An empty configuration indicates that the model is fine-tuned on the train dataset and evaluated on the test dataset (RQ1). "GRL" indicates models fine-tuned with the train dataset as the source and the test dataset as the target in an adversarial fashion (RQ2). "Silver" indicates models trained with silver summaries of the target (test) dataset (RQ3). "CS" and "MMR" represent CaseSummarizer and MMR unsupervised algorithms, from which the target silver summaries are derived.}
\scalebox{0.9}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\textbf{}}                                                                             & \textbf{Test \textrightarrow}               & \textbf{UK-Abs}      & \textbf{IN-Abs}      & \textbf{BVA-Ext}         \\ \hline
\multicolumn{2}{|c|}{\hspace{0.5cm}\textbf{Model Config}\hspace{0.5cm}}                                                                           & \hspace{0.04cm}\textbf{Train \textdownarrow} \hspace{0.04cm}         & \hspace{0.3cm}\textbf{R-1/R-2/R-L}\hspace{0.3cm} & \hspace{0.3cm}\textbf{R-1/R-2/R-L}\hspace{0.3cm} & \hspace{0.3cm}\textbf{R-1/R-2/R-L}\hspace{0.3cm} \\ \hline
\multicolumn{1}{|c|}{\multirow{12}{*}{BART}}                                                     &             & \multirow{4}{*}{UK-Abs} & 0.627/0.272/0.543    & 0.608/0.311/0.522    & 0.555/0.334/0.340    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & -                    & 0.614/0.316/0.526    & 0.553/0.336/0.460    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & -                    & 0.595/0.281/0.498    & 0.554/0.338/0.467    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & -                    & 0.597/0.290/0.507    & 0.556/0.342/0.476    \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{4}{*}{IN-Abs} & 0.615/0.255/0.532    & 0.625/0.337/0.548    & 0.481/0.226/0.306    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.620/0.264/0.536    & -                    & 0.524/0.294/0.440    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.610/0.253/0.525    & -                    & 0.562/0.372/0.491    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & 0.608/0.242/0.529    & -                    & 0.551/0.342/0.470    \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{4}{*}{BVA}    & 0.598/0.242/0.519    & 0.581/0.277/0.503    & 0.605/0.435/0.472    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.604/0.243/0.544    & 0.581/0.278/0.513    & -                    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.608/0.248/0.523    & 0.582/0.281/0.511    & -                    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & 0.606/0.245/0.525    & 0.585/0.284/0.512    & -                    \\ \hline
\multicolumn{1}{|c|}{\multirow{12}{*}{\begin{tabular}[c]{@{}c@{}}BERT-\\ BART\end{tabular}}}     &             & \multirow{4}{*}{UK-Abs} & 0.615/0.260/0.529    & 0.600/0.305/0.513    & 0.552/0.334/0.342    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & -                    & 0.607/0.308/0.522    & 0.554/0.336/0.461    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & -                    & 0.598/0.296/0.508    & 0..555/0.339/0.468   \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & -                    & 0.595/0.291/0.505    & 0.556/0.343/0.477    \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{4}{*}{IN-Abs} & 0.599/0.244/0.515    & 0.620/0.330/0.541    & 0.482/0.229/0.308    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.604/0.251/0.520    & -                    & 0.523/0.293/0.440    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.598/0.248/0.518    & -                    & 0.564/0.373/0.493    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & 0.596/0.246/0.516    & -                    & 0.555/0.362/0.465    \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{4}{*}{BVA}    & 0.590/0.235/0.508    & 0.580/0.279/0.501    & 0.602/0.427/0.465    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.595/0.238/0.522    & 0.575/0.270/0.502    & -                    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.598/0.241/0.527    & 0.578/0.272/0.500    & -                    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & 0.596/0.240/0.524    & 0.585/0.278/0.499    & -                    \\ \hline
\multicolumn{1}{|c|}{\multirow{12}{*}{\begin{tabular}[c]{@{}c@{}}Legal-\\ Pegasus\end{tabular}}} &             & \multirow{4}{*}{UK-Abs} & 0.624/0.271/0.541    & 0.615/0.323/0.532    & 0.528/0.308/0.451    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & -                    & 0.611/0.297/0.524    & 0.485/0.242/0.394    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & -                    & 0.611/0.313/0.527    & 0.537/0.315/0.458                  \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & -                    & 0.608/0.309/0.526    & 0.546/0.329/0.469    \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{4}{*}{IN-Abs} & 0.617/0.259/0.533    & 0.629/0.342/0.547    & 0.518/0.292/0.434    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.609/0.235/0.528    & -                    & 0.403/0.154/0.326    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.622/0.253/0.536    & -                    & 0.532/0.312/0.446    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & 0.619/0.251/0.534    & -                    & 0.546/0.335/0.465    \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{4}{*}{BVA}    & 0.596/0.247/0.522    & 0.601/0.303/0.522    & 0.603/0.424/0.453    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.599/0.235/0.517    & 0.609/0.301/0.523    & -                    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.609/0.245/0.524    & 0.598/0.297/0.518    & -                    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & 0.603/0.246/0.522    & 0.597/0.295/0.513    & -                    \\ \hline
\end{tabular}}
\end{table*}

==> text/tab-RQ2-3v3.tex <==
\begin{table*}[!ht]
\centering
\caption{ROUGE-L F-score (R-L) and BERT Score (BS) of three abstractive models trained under various configurations. Each target (test) dataset is represented by a column, while the source (train) is presented in the Source column. An empty configuration indicates that the model is fine-tuned on the source dataset and evaluated on the target dataset (RQ1). GRL indicates models fine-tuned in an adversarial fashion (RQ2). Silver indicates models trained with silver summaries of the target dataset (RQ3). CS and MMR represent CaseSummarizer and MMR unsupervised algorithms, from which the target silver summaries are derived. %\sg{In a very large majority of cases, Silver(MMR) gives better scores. Do we need to report Silver(CS) at all? We can just write in the text that we tried out multiple unsupervised summarization methods, and found MMR silver summaries to give the best results; hence reporting that only.} 
\textcolor{cyan}{\textbf{EDIT : New variants added table 8. 9. we can pick whichever appears good. (I prefer table 9)}. \sg{I see Table 9 is more compact, saves space, so fine. }}
}
\scalebox{0.9}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\textbf{}}                                                                             & \textbf{Target \textrightarrow}               & \textbf{UK-Abs}      & \textbf{IN-Abs}      & \textbf{BVA-Ext}         \\ \hline
\multicolumn{2}{|c|}{\hspace{1cm}\textbf{Model Config}\hspace{1cm}}                                                                           & \hspace{0.15cm}\textbf{Source \textdownarrow} \hspace{0.15cm}         & \hspace{0.55cm}\textbf{R-L/BS}\hspace{0.55cm} & \hspace{0.55cm}\textbf{R-L/BS}\hspace{0.55cm} & \hspace{0.55cm}\textbf{R-L/BS}\hspace{0.55cm} \\ \hline
\multicolumn{1}{|c|}{\multirow{12}{*}{\hspace{0.15cm}BART \hspace{0.15cm}}}                                                     &             & \multirow{4}{*}{UK-Abs} & 0.543/0.844     & 0.522/0.847     & 0.341/0.842     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           &  \hspace{0.75cm}GRL\hspace{0.75cm}         &                         & -               & 0.526/0.848     & 0.460/0.868     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & -               & 0.498/0.828     & 0.467/0.869     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & -               & 0.507/0.832     & 0.471/0.872     \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{4}{*}{IN-Abs} & 0.532/0.837     & 0.548/0.851     & 0.306/0.834     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.536/0.838     & -               & 0.440/0.864     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.525/0.833     & -               & 0.470/0.871     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & 0.529/0.838     & -               & 0.471/0.871     \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{4}{*}{BVA}    & 0.519/0.835     & 0.503/0.840     & 0.472/0.881     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.543/0.837     & 0.513/0.842     & -               \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.544/0.839     & 0.514/0.842     & -               \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & 0.546/0.839     & 0.515/0.842     & -               \\ \hline
\multicolumn{1}{|c|}{\multirow{12}{*}{\begin{tabular}[c]{@{}c@{}}BERT-\\ BART\end{tabular}}}     &             & \multirow{4}{*}{UK-Abs} & 0.529/0.845     & 0.513/0.846     & 0.342/0.842     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & -               & 0.522/0.848     & 0.461/0.868     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & -               & 0.505/0.834     & 0.464/0.868     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & -               & 0.508/0.838     & 0.465/0.868     \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{4}{*}{IN-Abs} & 0.515/0.838     & 0.541/0.851     & 0.308/0.836     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.520/0.838     & -               & 0.440/0.857     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.518/0.838     & -               & 0.463/0.869     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & 0.516/0.838     & -               & 0.465/0.869     \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{4}{*}{BVA}    & 0.508/0.837     & 0.501/0.839     & 0.465/0.880     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.522/0.838     & 0.504/0.840     & -               \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.524/0.838     & 0.508/0.842     & -               \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & 0.527/0.838     & 0.509/0.843     & -               \\ \hline
\multicolumn{1}{|c|}{\multirow{12}{*}{\begin{tabular}[c]{@{}c@{}}Legal-\\ Pegasus\end{tabular}}} &             & \multirow{4}{*}{UK-Abs} & 0.541/0.838     & 0.532/0.847     & 0.451/0.861     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & -               & 0.524/0.838     & 0.394/0.829     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & -               & 0.526/0.842     & 0.458/0.864     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & -               & 0.527/0.838     & 0.469/0.868     \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{4}{*}{IN-Abs} & 0.533/0.836     & 0.547/0.850     & 0.434/0.854     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.528/0.834     & -               & 0.326/0.818     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.536/0.836     & -               & 0.446/0.857     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & 0.534/0.836     & -               & 0.465/0.862     \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{4}{*}{BVA}    & 0.522/0.834     & 0.522/0.842     & 0.473/0.878     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.517/0.828     & 0.521/0.842     & -               \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.522/0.835     & 0.522/0.844     & -               \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver(MMR) &                         & 0.524/0.835     & 0.524/0.844     & -               \\ \hline
\end{tabular}}
\end{table*}

==> text/tab-RQ2-3v4.tex <==
\begin{table*}[!ht]
\centering
\caption{ROUGE-L F-score (R-L) and BERT Score (BS) of three abstractive models trained under various configurations. Each target (test) dataset is represented by a column, while the source (train) is presented in the Train column. An empty configuration indicates that the model is fine-tuned on the source dataset and evaluated on the target dataset (RQ1). GRL indicates models fine-tuned in an adversarial fashion (RQ2). Silver indicates models trained with silver summaries of the target dataset obtained through unsupervised MMR algorithm (RQ3). %"CS" and "MMR" represent CaseSummarizer and MMR unsupervised algorithms, from which the target silver summaries are derived. %\sg{In a very large majority of cases, Silver gives better scores. Do we need to report Silver(CS) at all? We can just write in the text that we tried out multiple unsupervised summarization methods, and found MMR silver summaries to give the best results; hence reporting that only.}
}
\scalebox{0.9}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\textbf{}}                                                                             & \textbf{Test \textrightarrow}               & \textbf{UK-Abs}      & \textbf{IN-Abs}      & \textbf{BVA-Ext}         \\ \hline
\multicolumn{2}{|c|}{\textbf{Model Config}}                                                                           & \hspace{0.15cm}\textbf{Train \textdownarrow} \hspace{0.15cm}         & \hspace{0.55cm}\textbf{R-L/BS}\hspace{0.55cm} & \hspace{0.55cm}\textbf{R-L/BS}\hspace{0.55cm} & \hspace{0.55cm}\textbf{R-L/BS}\hspace{0.55cm} \\ \hline
\multicolumn{1}{|c|}{\multirow{9}{*}{\hspace{0.25cm}BART \hspace{0.25cm}}}                                                     &             & \multirow{3}{*}{UK-Abs} & -    & 0.522/0.847     & 0.341/0.842     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           &  \hspace{0.5cm}GRL\hspace{0.5cm}         &                         & -               & \textbf{0.526}/\textbf{0.848}     & 0.460/0.868     \\ \cline{2-2} \cline{4-6} 
%\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & -               & 0.498/0.828     & 0.467/0.869     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver &                         & -               & 0.507/0.832     & \textbf{0.471/0.872}     \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{3}{*}{IN-Abs} & 0.532/0.837     & -    & 0.306/0.834     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & \textbf{0.536/0.838}     & -               & 0.440/0.864     \\ \cline{2-2} \cline{4-6} 
%\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.525/0.833     & -               & 0.470/0.871     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver &                         & 0.529/0.838     & -               & \textbf{0.471/0.871}    \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{3}{*}{BVA}    & 0.519/0.835     & 0.503/0.840     & -     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.543/0.837     & 0.513/0.842     & -               \\ \cline{2-2} \cline{4-6} 
%\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.544/0.839     & 0.514/0.842     & -               \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver &                         & \textbf{0.546/0.839}     & \textbf{0.515/0.842}     & -               \\ \hline
\multicolumn{1}{|c|}{\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}BERT-\\ BART\end{tabular}}}     &             & \multirow{3}{*}{UK-Abs} & -     & 0.513/0.846     & 0.342/0.842     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & -               & \textbf{0.522/0.848}     & 0.461/0.868     \\ \cline{2-2} \cline{4-6} 
%\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & -               & 0.505/0.834     & 0.464/0.868     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver &                         & -               & 0.508/0.838     & \textbf{0.465/0.86}8     \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{3}{*}{IN-Abs} & 0.515/0.838     & -    & 0.308/0.836     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & \textbf{0.520/0.838}     & -               & 0.440/0.857     \\ \cline{2-2} \cline{4-6} 
%\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.518/0.838     & -               & 0.463/0.869     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver &                         & 0.516/0.838     & -               & \textbf{0.465/0.869}     \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{3}{*}{BVA}    & 0.508/0.837     & 0.501/0.839     & -    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.522/0.838     & 0.504/0.840     & -               \\ \cline{2-2} \cline{4-6} 
%\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.524/0.838     & 0.508/0.842     & -               \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver &                         & \textbf{0.527/0.838}     & \textbf{0.509/0.843}     & -               \\ \hline
\multicolumn{1}{|c|}{\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}Legal-\\ Pegasus\end{tabular}}} &             & \multirow{3}{*}{UK-Abs} & -     & \textbf{0.532/0.847}     & 0.451/0.861     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & -               & 0.524/0.838     & 0.394/0.829     \\ \cline{2-2} \cline{4-6} 
%\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & -               & 0.526/0.842     & 0.458/0.864     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver &                         & -               & 0.527/0.838     & \textbf{0.469/0.868}     \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{3}{*}{IN-Abs} & 0.533/0.836     & -    & 0.434/0.854     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.528/0.834     & -               & 0.326/0.818     \\ \cline{2-2} \cline{4-6} 
%\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.536/0.836     & -               & 0.446/0.857     \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver &                         & \textbf{0.534/0.836}     & -               & \textbf{0.465/0.862}     \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                                                                           &             & \multirow{3}{*}{BVA}    & 0.522/0.834     & 0.522/0.842     & -    \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & GRL         &                         & 0.517/0.828     & 0.521/0.842     & -               \\ \cline{2-2} \cline{4-6} 
%\multicolumn{1}{|c|}{}                                                                           & Silver (CS) &                         & 0.522/0.835     & 0.522/0.844     & -               \\ \cline{2-2} \cline{4-6} 
\multicolumn{1}{|c|}{}                                                                           & Silver &                         & \textbf{0.524/0.835}     & \textbf{0.524/0.844}     & -               \\ \hline
\end{tabular}}
\label{RQ2-3}
\end{table*}

==> text/tab-RQ2-3v5.tex <==

\begin{table*}[!ht]
\centering
\caption{ROUGE-L F-score (R-L) and BERT Score (BS) of three abstractive models trained under various configurations. Each target (test) dataset is represented by a column, while the corresponding source (train) is presented in the S column. An empty configuration indicates that the model is fine-tuned on the source dataset and evaluated on the target dataset (RQ1). GRL indicates models fine-tuned in an adversarial fashion (RQ2). Silver indicates models trained with silver summaries of the target dataset (RQ3). CS and MMR represent CaseSummarizer and MMR unsupervised algorithms, from which the target silver summaries are derived. %\sg{In a very large majority of cases, Silver(MMR) gives better scores. Do we need to report Silver(CS) at all? We can just write in the text that we tried out multiple unsupervised summarization methods, and found MMR silver summaries to give the best results; hence reporting that only.}
}
\scalebox{0.9}{
\begin{tabular}{|cc|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{}                               & \textbf{Target   \textrightarrow}   &                         & \textbf{UK-Abs}      &                         & \textbf{IN-Abs}      &                         & \textbf{BVA-Ext}         \\ \hline
\multicolumn{2}{|c|}{\textbf{Model Config}}                                        & \hspace{0.15cm}\textbf{S} \hspace{0.15cm}                      & \hspace{0.55cm}\textbf{R-L/BS} \hspace{0.55cm}     & \hspace{0.15cm}\textbf{S}\hspace{0.15cm}                       & \hspace{0.55cm}\textbf{R-L/BS}\hspace{0.55cm}      & \hspace{0.15cm}\textbf{S} \hspace{0.15cm}                      & \hspace{0.55cm}\textbf{R-L/BS}\hspace{0.55cm}      \\ \hline
\multicolumn{1}{|c|}{\multirow{8}{*}{\hspace{0.15cm}BART \hspace{0.15cm}}}  &             & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{IN-Abs}}} & 0.532/0.837 & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{UK-Abs}}} & 0.522/0.847 & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{UK-Abs}}} & 0.341/0.842 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & GRL         &                         & \textbf{0.536/0.838} &                         & \textbf{0.526/0.848} &                         & 0.460/0.868 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & Silver (CS) &                         & 0.525/0.833 &                         & 0.498/0.828 &                         & 0.467/0.869 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & Silver(MMR) &                         & 0.529/0.838 &                         & 0.507/0.832 &                         & \textbf{0.471/0.872} \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                               &             & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{BVA-Ext}}}   & 0.519/0.835 &\multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{BVA-Ext}}}    & 0.503/0.840 & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{IN-Abs}}} & 0.306/0.834 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & GRL         &                         & 0.544/0.837 &                         & 0.513/0.842 &                         & 0.440/0.864 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & Silver (CS) &                         & 0.543/0.839 &                         & 0.514/0.842 &                         & 0.470/0.871 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & Silver(MMR) &                         & \textbf{0.546/0.839} &                         & \textbf{0.515/0.842} &                         & \textbf{0.471/0.871} \\ \hline
\multicolumn{1}{|c|}{\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}BERT-\\ BART\end{tabular}}}     &             & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{IN-Abs}}} & 0.515/0.838 & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{UK-Abs}}} & 0.513/0.846 & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{UK-Abs}}} & 0.342/0.842 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & GRL         &                         & \textbf{0.520/0.838} &                         & \textbf{0.522/0.848} &                         & 0.461/0.868 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & Silver (CS) &                         & 0.518/0.838 &                         & 0.505/0.834 &                         & 0.464/0.868 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & Silver(MMR) &                         & 0.516/0.838 &                         & 0.508/0.838 &                         & \textbf{0.465/0.868} \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                               &             & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{BVA-Ext}}}  & 0.508/0.837 & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{BVA-Ext}}}    & 0.501/0.839 & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{IN-Abs}}} & 0.308/0.836 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & GRL         &                         & 0.522/0.838 &                         & 0.504/0.840 &                         & 0.440/0.857 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & Silver (CS) &                         & 0.524/0.838 &                         & 0.508/0.842 &                         & 0.463/0.869 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & Silver(MMR) &                         & \textbf{0.527/0.838} &                         & \textbf{0.509/0.843} &                         & \textbf{0.465/0.869} \\ \hline
\multicolumn{1}{|c|}{\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Legal-\\ Pegasus\end{tabular}}}  &             & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{IN-Abs}}} & 0.533/0.836 & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{UK-Abs}}} & 0.532/0.847 & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{UK-Abs}}} & 0.451/0.861 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & GRL         &                         & 0.528/0.834 &                         & 0.524/0.838 &                         & 0.394/0.829 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & Silver (CS) &                         & \textbf{0.536/0.836} &                         & 0.526/0.842 &                         & 0.458/0.864 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & Silver(MMR) &                         & 0.534/0.836 &                         & \textbf{0.527/0.838} &                         & \textbf{0.469/0.868} \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                               &             & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{BVA-Ext}}}   & 0.522/0.834 & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{BVA-Ext}}}    & 0.522/0.842 & \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{IN-Abs}}} & 0.434/0.854 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & GRL         &                         & 0.517/0.828 &                         & 0.521/0.842 &                         & 0.326/0.818 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & Silver (CS) &                         & 0.522/0.835 &                         & 0.522/0.844 &                         & 0.446/0.857 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{}                               & Silver(MMR) &                         & \textbf{0.524/0.835} &                         & \textbf{0.524/0.844} &                         & \textbf{0.465/0.862} \\ \hline
\end{tabular}}
\end{table*}
